Shared lightweight autonomous vehicles for urban food deliveries: A simulation study

In recent years, the rapid growth of on-demand deliveries, especially in food deliveries, has spurred the exploration of innovative mobility solutions. In this context, lightweight autonomous vehicles have emerged as a potential alternative. However, their fleet-level behavior remains largely unexplored. To address this gap, we have developed an agent-based model and an environmental impact study assessing the fleet performance of lightweight autonomous food delivery vehicles. This model explores critical factors such as fleet sizing, service level, operational strategies, and environmental impacts. We have applied this model to a case study in Cambridge, MA, USA, where results indicate that there could be environmental benefits in replacing traditional car-based deliveries with shared lightweight autonomous vehicle fleets. Lastly, we introduce an interactive platform that offers a user-friendly means of comprehending the model's performance and potential trade-offs, which can help inform decision-makers in the evolving landscape of food delivery innovation.

==> letter.tex <==
October 27, 2023
Transportation Research Part D: Transport and Environment


Dear Guest Editors of the Special Issue on 'Zero-Emission Mobility Strategies: Innovation, Diversity, and Integration',

We hope this letter finds you well. We writing to present our research paper, "Lighweight autonomous vehicles for food deliveries: A simulation study", authored by Ainhoa Genua Cerviño, Naroa Coretti Sanchez, Elaine Liu Wang, Arnaud Grignard, and Kent Larson, for publication in the esteemed journal Transportation Research Part D: Transport and Environment. Our paper delves into the realm of innovative solutions within the domain of on-demand food delivery, particularly focusing on lightweight autonomous vehicles.

In recent years, the rapid growth of on-demand deliveries, especially in the food delivery sector, has spurred the exploration of innovative mobility solutions. In this context, lightweight autonomous vehicles have emerged as a potential alternative. However, their fleet-level behavior remains largely unexplored. To address this critical gap in the literature, we have developed an agent-based model and conducted an environmental impact study to assess the fleet performance of lightweight autonomous vehicles in the context of food delivery.

Our model explores essential factors such as fleet sizing, service levels, operational strategies, and environmental impacts, providing a comprehensive understanding of the dynamics at play. We have applied this model in a real-world case study set in Cambridge, MA, USA. The results of our study indicate that there could be environmental benefits in replacing traditional car-based deliveries with shared lightweight autonomous vehicle fleets. 

Furthermore, we introduce an interactive platform designed to make the model's outcomes accessible and comprehensible for stakeholders. This user-friendly platform facilitates a deeper understanding of the model's performance and potential trade-offs, offering valuable insights for decision-makers in the continually evolving landscape of food delivery innovation.

We believe that our research contributes to the ongoing dialogue on the sustainability and efficiency of emerging solutions in the field of on-demand food delivery services. It addresses not only the technological aspect but also the environmental and operational dimensions of these innovative solutions. 

We confirm the originality of this work, which has not been published elsewhere, nor is it currently under consideration for publication elsewhere. Furthermore, we declare that there are no conflicts of interest to disclose. I, Naroa Coretti Sanchez, will serve as the corresponding author and can be readily contacted at naroa@mit.edu for all correspondence related to this manuscript.

We greatly appreciate your time and consideration. We look forward to the opportunity to contribute to the distinguished Transportation Research Part D: Transport and Environment journal.

Sincerely,

Naroa Coretti Sánchez
naroa@mit.edu
MIT Media Lab – City Science
20 Amets Street, E15-368 Cambridge, MA, USA





==> mobi-draft.tex <==
\section{MoBi: A decision-making support tool for multi-stakeholder scenarios}
\label{sec:Tangible interface}

Having discussed all the outcomes extracted from the agent-based simulation study presented in this article, it is concluded that all the results could be very interesting for a wide variety of stakeholders, including food delivery companies, policymakers, design engineers, and so on. For this reason, as the last step of the study, a multi-stakeholder interactive decision-making tool called MoBi has been deployed as presented in Figure \ref{fig:Setup and displays}.

\begin{figure}[!h]
    \centering
    \caption{Set-up, displays, and interaction panels of MoBi, a multi-stakeholder interactive decision-making tool for food deliveries.\centering}
    \includegraphics[width=0.5\linewidth]{figures/Setup and displays.jpg}
    \label{fig:Setup and displays}
\end{figure}

MoBi is an interactive platform to support diverse stakeholders in building consensus in decision-making processes. This tool is dynamically linked to the simulation model described in this thesis so that stakeholders can interact with it and see the impacts of their choices in real time. Such interactions can help stakeholders understand each other’s perspectives and trade-offs and make better decisions around future mobility systems' design, development, and deployment. Moreover, this tool is easily adaptable to any city or use case scenario that wants to be analyzed.

\subsection{MoBi setup and deployment}

Currently, this platform stands at the entrance of the MIT Media Lab City Science research group as part of the demo space. The parts needed for the deployment are a computer (with GAMA, mouse, and keyboard), a screen (TV), a projector, a table, Lego blocks, an Arduino board, sliders, buttons, and wires.

This real-time interactive simulation has been programmed in GAMA due to its advanced display modes. The display of the program is divided into two main visualizations (indicators display on the TV screen and dynamic map display over the table through the projector). At the same time, GAMA is connected to Arduino and reads the state of the buttons and sliders that define the interactions in real-time.

\subsubsection{Interactive board}
\label{subsubsection: Interactive board}

The users engage with the model through a custom-made interactive board. This board gives the users access to decide which scenario they are willing to visualize as well as the chance to design their own autonomous micro-mobility fleet system with customized vehicle configurations and charging operational strategies. This board is formed by four buttons and two sliders (see Figure \ref{fig:Current scenario interacions} and Figure \ref{fig:Future scenario interacions}) that allow the interactions described in Figure \ref{fig:Interactions}.

\begin{figure}[!h]
    \begin{floatrow} 
        \ffigbox[7cm]{%
            \includegraphics[width=0.45\textwidth]{figures/Current Scenario Interaction.jpg}
        }{%
          \captionsetup{width=1.15\linewidth}
          \caption{Interactions that the user can explore in the current car-based scenario.\centering}%
          \label{fig:Current scenario interacions}
        }
       \ffigbox[7cm]{%
            \includegraphics[width=0.45\textwidth]{figures/Future Scenario Interaction.jpg}
        }{%
          \captionsetup{width=1.15\linewidth}
          \caption{Interactions that the user can explore in the future autonomous micro-mobility-based scenario.\centering}%
          \label{fig:Future scenario interacions}
        }
    \end{floatrow}
\end{figure}

\begin{figure}[!h]
    \centering
    \caption{Schema with the interactions that the user can explore in MoBi.\centering}
    \includegraphics[width=0.75\linewidth]{figures/Interactions.png}
    \label{fig:Interactions}
\end{figure}

As presented in Figure \ref{fig:Current scenario interacions} and Figure \ref{fig:Interactions}, the user can select the baseline current car-based scenario to understand how the food deliveries are currently handled in the visualization area. In this scenario, the user can switch to the electrification of the fleet and notice the impacts of this decision. In the future scenario where autonomous micro-mobility vehicles are used for food deliveries, users can explore more interactions (Figure \ref{fig:Future scenario interacions} and Figure \ref{fig:Interactions}). The idea is that the people interacting with the table get the chance to design the vehicles as they desire and understand the implications that their decisions may carry with them. For this reason, the users are able to choose between conventional and fast charging operational strategies and also play with the vehicle configurations studied in this paper (small or large battery sizes, 60 – 300 fleet size, and 6 – 20 km/h driving speed).

\subsubsection{Indicators display}

This display aims to provide different insides to the users (Figure \ref{fig:Indicators display}) by plotting several indicators divided into four main categories.

\begin{figure}[!h]
    \centering
    \caption{Information on the scenario (1 – red), environmental impacts (2 – green), service level (3 – blue), and fleet performance (4 – yellow) display that the user needs to analyze to generate insights.\centering}
    \includegraphics[width=0.6\linewidth]{figures/Indicators Display.jpg}
    \label{fig:Indicators display}
\end{figure}

The first section of the display (Figure \ref{fig:Indicators display} – 1) corresponds to an informative category showing the title of the project, “Autonomous micro-mobility for food deliveries,” and the scenario visualized (“Current scenario: Cars” vs. “Future scenario: Autonomous micro-mobility”).

The second section (Figure \ref{fig:Indicators display} – 2) concerns the environmental impacts of the analyzed food delivery fleet configuration. This section includes just one display which consists of a dynamic horizontal bar chart that shows the grams of CO2 per vehicle kilometer traveled by the selected system. Every time the user makes an update by pressing the buttons or moving the sliders, the value of this bar is updated. In all cases, the emissions of both current car-based food deliveries are always displayed so that the user can see those baselines as a reference value.

The third section (Figure \ref{fig:Indicators display} – 3) shows the service level-related indicators.

\begin{itemize}
    \item First, a chart plots the average wait time of the food delivery orders, representing the time elapsed from the moment they are placed to the moment they arrive at their destination. This display keeps updating in real simulation time and consists of a moving window that displays the results of the last 12 hours. This display allows the user to understand if the proposed configuration meets the established quality standard stating that 95\% of the trips must be accomplished in less than 40 minutes.
    \item Second, there is a counter that shows the number of unserved orders that are taking place in the analyzed scenario. In opposition to how the main study of this research has been done in which all of the trips needed to be served for the analysis, a maximum wait time has been set for this interactive tool. This limit has been set at the considered maximum wait time of 40 minutes. It has been added to avoid a potential slowing down of the simulation due to an overload of information. This counter resets every time the user interacts with the model so that only the orders unserved under a specific configuration are displayed.
\end{itemize}

The fourth and last section (Figure \ref{fig:Indicators display} – 4) presents vehicles' real-time activities. Similar to the average wait time plot, this is a real-time updated plot that displays the results of the last 12 hours of the simulation. In this case, the number of vehicles fulfilling different tasks is displayed (idle, pick up or delivery, and charging). This display is added to give the user an idea of why a system configuration may not work. 

\subsubsection{Dynamic map}

This last display consists of the visualization of the case study area map, the movement of the agents on the roads, and the visualization of the main activities that are taking place in the simulation. This dynamic display updates in real simulation time and is projected over a Lego table, as shown in Figure \ref{fig:Map display}.

\begin{figure}[!h]
    \centering
    \caption{Interactive board (1 – red), legend (2 – green), road network (3 – blue), and agents (4 – yellow) displays that the user needs to analyze to generate insights.\centering}
    \includegraphics[width=0.75\linewidth]{figures/Map Display.jpg}
    \label{fig:Map display}
\end{figure}

Different layers form the display:
\begin{itemize}
    \item The interactive board explained in Section \ref{subsubsection: Interactive board} is at the bottom left of the table (Figure {fig:Map display} – 1).
    \item A legend explaining the visualizations is placed at the bottom of the table to the right of the interactive board (Figure {fig:Map display} – 2). This legend does not only include the explanation of the different moving agents and the different states but also the visualization of the scenario the user has chosen and the timestamp of the day.
    \item Through GIS data, GAMA can define the city road network where the agents will move. In this case, the visualization area encompasses part of Cambridge plus a small part of Somerville (Figure {fig:Map display} – 3).
    \item The movement of the different agents in the simulation is visualized over the road network (Figure {fig:Map display} – 4). In particular, the user is able to visualize cars (in blue) or autonomous micro-mobility vehicles (in green) idling (static arrows), picking up food delivery orders (moving arrows), delivering orders (moving arrows with a bright circle), going to charge (red moving arrows), and charging (static red arrows). Moreover, the user is also able to identify the food delivery orders in two of their states: food delivery orders waiting for a vehicle assignation (in red) and food delivery orders being delivered (bright circle that moves over the vehicle). Furthermore, the gas/charging stations are also visualized (purple hexagon). In fact, their size changes depending on how many vehicles are hosted simultaneously.
\end{itemize}

\subsection{MoBi use-cases}

This platform aims to facilitate the design and implementation of new mobility systems for a positive impact in the cities of the future through a simple-to-use tool. For this reason, it has already been used in diverse circumstancex.

First, it was presented platform was presented to some members of the Council of Gipuzkoa, the director of the MUBIL Foundation, and the dean and development director of Tecnun – School of Engineering (Spain). On this occasion, the stakeholders showed a clear interest in the tool and found it very useful.

Second, the tool was displayed at the MIT Media Lab Members' Event on April 2023. Through this event, the tool was presented to diverse Media Lab member companies and researchers. The tool caught people's attention and encouraged them to interact with it, generating engaging conversations and powerful insights. Moreover, as part of the event, the tool was also live-streamed for online members.

Currently, the tool is still being displayed at the MIT City Science demo space, and it is frequently shown as part of private tours of diverse Media Lab stakeholders.

==> notes-draft.tex <==
% Pop growth mainly urban --> Macro cities. Poses many challenges . One of them is sustainable mobility modes for people and goods.

%In addition, urban mobility demand is increasing. One of the factors increasing per capita mobility demand is ecommerce. 
%Evolution of ecommerce (highlight previous growth trends,  and how they increased with the pandemic).
%There was an increase trend that was already there but that has been accelerated by COVID-19. 




% Another approach is to take advantage of the off-peak availability of shared autonomous micro-mobility vehicles (bicycles, tricycles) used as mobility on demand system for people \cite{our work}. During rush hour these vehicles can move people. Off peak they can do other tasks such as food delivery.

\medskip


%The MIT Media Lab City Science research group proposes two different shared autonomous micro-mobility vehicles, the MIT Autonomous Bicycle \cite{sanchez2020autonomous}, and the Persuasive Electric Vehicle (PEV) \cite{lin2021affordable}, for the movement of people. Previous studies \cite{sanchez2022performance,sanchez2022simulation} show that fleet sizing for autonomous mobility on-demand is largely dependent on the peak of demand during the morning and evening rush hours. These results indicate that these systems have spare capacity to accomplish other tasks. For this reason, we are aiming to study their potential multi-functionality by understanding their performance for food deliveries.}
\medskip

%% Para cerrar esta sección yo diría que aunque estas soluciones se estén planteando, no hay ningún estudio que se centre en ver su performance a nivel de flota, y que esto es imprescindible para saber qué comportamiento van a tener, que impactos van a generar etc.  (Luego vas a desarrollar más esto en el Conribution, pero está bien mencionarlo aquí)

% REVIEW what has been done in fleet analysis of autonomous vehicles for food delivery!
% If there isn't anything, is there something for package delivery?
% - There is for package delivery but not food?
% - Why is this one different? Different demand characteristics and requirements? (Most of the demand at lunch time, the maximum wait time is related to food becoming cold...)
% Write found articles and a sentence that describes each


%These new vehicles could help to address the growing demand while transitioning to lighter vehicles that could be better suited to deliver small food packages than heavy, full-sized cars. Ideally, these vehicles could be able to cover food delivery demand at a lower economic and environmental cost. Moreover, these lightweight vehicles are designed to operate in sidewalks or bike lanes, avoiding the need for additional road space in cities \citep{poeting2019simulation}.  Overall, this approach seems promising at least from a conceptual standpoint.
